Secure Software/Hardware Hybrid In-Field Testing for System-on-Chip

Modern Systems-on-Chip (SoCs) incorporate built-in self-test (BIST) modules deeply integrated into the device's intellectual property (IP) blocks. Such modules handle hardware faults and defects during device operation. As such, BIST results potentially reveal the internal structure and state of the device under test (DUT) and hence open attack vectors. So-called result compaction can overcome this vulnerability by hiding the BIST chain structure but introduces the issues of aliasing and invalid signatures. Software-BIST provides a flexible solution, that can tackle these issues, but suffers from limited observability and fault coverage. In this paper, we hence introduce a low-overhead software/hardware hybrid approach that overcomes the mentioned limitations. It relies on (a) keyed-hash message authentication code (KMAC) available on the SoC providing device-specific secure and valid signatures with zero aliasing and (b) the SoC processor for test scheduling hence increasing DUT availability. The proposed approach offers both on-chip- and remote-testing capabilities. We showcase a RISC-V-based SoC to demonstrate our approach, discussing system overhead and resulting compaction rates.

==> Acknowledgments.tex <==
%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.

\begin{acks}
This work was supported by VE-Jupiter (16ME0231K, 16ME0233, 16ME0234) %
and KI-IoT (16ME0091K)%
, funded by the Federal Ministry of Education and Research (BMBF).
%This work has been funded by public third-party funding. Details are omitted for blind review.
\end{acks}

==> tables/iscas85_results_sha3_224.tex <==
\begin{table}[ht]
\centering
\caption{Compaction \& Aliasing Rate Analysis utilizing ISCAS-85 Benchmark}
\resizebox{.5\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\textbf{}      & \textbf{\begin{tabular}[c]{@{}c@{}}Primary\\ Outputs\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# Test\\ Pattern\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Test Response\\ Length\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Compaction\\ Rate\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Aliasing\\ Rate\end{tabular}} \\ \hline
\textbf{c17}   & 2                                                                  & 7                                                                  & 14                                                                      & -1500$\%$                                                          & 0$\%$                                                            \\
\textbf{c432}  & 7                                                                  & 63                                                                 & 441                                                                     & 49.20$\%$                                                          & 0$\%$                                                            \\
\textbf{c499}  & 32                                                                 & 55                                                                 & 1760                                                                    & 87.27$\%$                                                          & 0$\%$                                                            \\
\textbf{c880}  & 26                                                                 & 148                                                                & 3848                                                                    & 94.18$\%$                                                          & 0$\%$                                                            \\
\textbf{c1355} & 32                                                                 & 100                                                                & 3200                                                                    & 93.00$\%$                                                          & 0$\%$                                                            \\
\textbf{c1908} & 25                                                                 & 128                                                                & 3200                                                                    & 93.00$\%$                                                          & 0$\%$                                                            \\
\textbf{c2670} & 140                                                                & 444                                                                & 62160                                                                   & 99.64$\%$                                                          & 0$\%$                                                            \\
\textbf{c3540} & 22                                                                 & 264                                                                & 5808                                                                    & 96.14$\%$                                                          & 0$\%$                                                            \\
\textbf{c5315} & 123                                                                & 599                                                                & 73677                                                                   & 99.69$\%$                                                          & 0$\%$                                                            \\
\textbf{c6288} & 32                                                                 & 33                                                                 & 1056                                                                    & 78.79$\%$                                                          & 0$\%$                                                            \\
\textbf{c7552} & 108                                                                & 455                                                                & 49140                                                                   & 99.54$\%$                                                          & 0$\%$                                                           
\end{tabular}
}
\label{tab:iscas85_results}
\end{table}

==> tables/sha3_overview.tex <==
\begin{table}[t]
\caption{Overview of SHA3 Hash Modes \cite{2015_sha3_nist_fips}}
\resizebox{.49\textwidth}{!}{
\begin{tabular}{c|c|c|c|c}
                   & \textbf{Hash Length $d$} & \textbf{Rate Size $r$} & \textbf{Capacity Size $c$} & \textbf{Collision} \\ \hline
\textbf{SHA-3-224} & 224                      & 1152                   & 448                        & 112                \\
\textbf{SHA-3-256} & 256                      & 1088                   & 512                        & 128                \\
\textbf{SHA-3-384} & 384                      & 832                    & 768                        & 192                \\
\textbf{SHA-3-512} & 512                      & 576                    & 1024                       & 256               
\end{tabular}
}
\label{tab:sha3_overview}
\end{table}
